Large Language Models are Interpretable Learners

The trade-off between expressiveness and interpretability remains a core challenge when building human-centric predictive models for classification and decision-making. While symbolic rules offer interpretability, they often lack expressiveness, whereas neural networks excel in performance but are known for being black boxes. In this paper, we show a combination of Large Language Models (LLMs) and symbolic programs can bridge this gap. In the proposed LLM-based Symbolic Programs (LSPs), the pretrained LLM with natural language prompts provides a massive set of interpretable modules that can transform raw input into natural language concepts. Symbolic programs then integrate these modules into an interpretable decision rule. To train LSPs, we develop a divide-and-conquer approach to incrementally build the program from scratch, where the learning process of each step is guided by LLMs. To evaluate the effectiveness of LSPs in extracting interpretable and accurate knowledge from data, we introduce IL-Bench, a collection of diverse tasks, including both synthetic and real-world scenarios across different modalities. Empirical results demonstrate LSP's superior performance compared to traditional neurosymbolic programs and vanilla automatic prompt tuning methods. Moreover, as the knowledge learned by LSP is a combination of natural language descriptions and symbolic rules, it is easily transferable to humans (interpretable), and other LLMs, and generalizes well to out-of-distribution samples.

==> 3_1_method_framework.tex <==
% \begin{itemize}
%     \item Using LLMs to write prompt
%         maybe move it to later, this way we can claim that the task is instruction induction, existing prompt 
%         (maybe move it to later, this way we can claim that the task is instruction induction, existing prompt optimization methods often perform instruction induction, we on the other hand prompt LLM to summarize rules, this performs better according to our ablation study)
% \end{itemize}

% \paragraph{Using LLM to optimize prompts}
% While current practice often involves manual prompt engineering to solve \eqref{eq.erm.prompt}, recent advances demonstrate that LLMs can reverse-engineer instructions from raw data and refine their responses iteratively.
% This process can be conceptualized as using LLMs as the optimizers (cite) to solve the objective in \eqref{eq.erm.prompt}.
% The LLM's inherit ability to serve as both the model and the optimizer in \eqref{eq.erm.prompt} enables us to implement a complete learning pipeline within the framework of pretrained LLMs, eliminating the need for any additional parameterization.
% In our work, we similarly employ the LLM-as-Optimizer approach when designing LLM-based Neurosymbolic Programs.


==> 3_1_method_framework_old.tex <==
\begin{itemize}
    \item Prompting LLM to model selection
    \item Prompt Optimization to ERM
    \item Using LLMs to write prompt
        maybe move it to later, this way we can claim that the task is instruction induction, existing prompt 
        (maybe move it to later, this way we can claim that the task is instruction induction, existing prompt optimization methods often perform instruction induction, we on the other hand prompt LLM to summarize rules, this performs better according to our ablation study)
\end{itemize}

Pretrained LLMs (Large Language Models) have demonstrated a remarkable capacity to understand and respond to natural language instructions, known as "prompts."
This ability allows them to tackle a wide range of tasks, including solving math problems, writing codes, visual recognition, knowledge retrieval, etc, which are historically handled by separated models.
While this interaction is often conceptualized as conversational, it can also be framed within traditional learning theory and directly linked to model selection.
This section explores the unification of LLM prompting, which will motivate using LLM to implement Neurosymbolic Programs that encode interpretable decision making process in Section~\ref{sec.method.algo}.


\paragraph{Re-imagine the role of prompts in LLM as accessing conditional probabilistic models}
We first show how prompting a pretrained LLM can be naturally viewed as sub-model selection.
LLMs pretrained on the next token prediction task model the following joint distribution of a sequence of tokens $\{w_i\}|_{i=1}^n$:
\begin{align}
    P(w_1, w_2, \ldots, w_n) = \prod_{i=1}^{n} P(w_i \mid w_1, w_2, \ldots, w_{i-1}) = f(w_i \mid w_1, w_2, \ldots, w_{i - 1}; \theta)
\end{align}
This equation expresses the probability of the entire sequence as the product of conditional probabilities, where each word $w_i$ is predicted given all the preceding tokens.
The conditional probability $P(w_i \mid w_1, w_2, \ldots, w_{i-1})$ is parameterized by an Auto-Regressive neural network (like the Transformer in GPT).
The goal of training is to minimize the negative log-likelihood:
\begin{align}
    \argmin_\theta \mathcal{L}(\theta) = -\sum_{t=1}^{T} \log P(w_t \mid w_1, w_2, \ldots, w_{t-1}; \theta)
\end{align}
After training, the model can be used by providing a prompt $t=\{w_1, w_2, \ldots, w_m\}$ to the model detailing the target task.
The key to connect this to traditional learning theory is to view the training process as optimizing a "SuperNet" of conditional probabilistic models (CPM).
Each CPM shares the same parameter $\theta$, but is uniquely defined by the sampled preceding tokens, aka prompts, $t = \{w_1, w_2, \ldots, w_{i - 1}\}$.
Therefore, after training, instead of obtaining one model, we obtained a set of conditional probabilistic models $P(w \mid t; \theta)$.
As a result, prompting LLM, agnostic to specific applications (Jailbreaking, Agent, RAG, QA, etc), can thus be viewed as selecting the appropriate sub-model from the SuperNet that best executes certain task.
Since the prompts that distinguish those models are written in nature language, the model selection process is inherently human-interpretable.


\paragraph{ERM and Hypothesis space defined by LLM submodels}
The selection problem of those submodels has a direct connect to the empirical risk minimization (ERM) framework.
Consider the task of learning a predictive function $\phi(x, \theta)$ to infer on a set of labeled examples ${(x_1, y_1), (x_2, y_2), ..., (x_n, y_n)}$, the ERM formulation can be written as:
\begin{align}
    \hat{f} = \arg \min_{f \in \mathcal{F}} \frac{1}{n} \sum_{i=1}^{n} \mathcal{L}(y_i, f(x_i)) + \lambda\mathcal{R}(f),
\end{align}
where $f$ is the learned model, $\mathcal{F}$ is the hypothesis space, $\mathcal{L}$ is the loss function and $\mathcal{R}$ is the regularization term.
If the hypothesis space is popularized by the submodels embedded in pretrained LLM, the objective becomes:
\begin{align}
    \hat{t} = \arg \min_{t \in \mathcal{T}} \frac{1}{n} \sum_{i=1}^{n} \mathcal{L}(y_i, P\big{[}\hat{y}_i|t\big{]}) + \lambda\mathcal{R}(t),
    \label{eq.erm.prompt}
\end{align}
where $t \in \mathcal{T}$ is the space of all prompts.
This demonstrates that carefully designing prompts for LLMs is fundamentally a process of model (hypothesis) selection.


\paragraph{Using LLM to optimize prompts}
While current practice often involves manual prompt engineering to solve \eqref{eq.erm.prompt}, recent advances demonstrate that LLMs can reverse-engineer instructions from raw data and refine their responses iteratively.
This process can be conceptualized as using LLMs as the optimizers (cite) to solve the objective in \eqref{eq.erm.prompt}.
The LLM's inherit ability to serve as both the model and the optimizer in \eqref{eq.erm.prompt} enables us to implement a complete learning pipeline within the framework of pretrained LLMs, eliminating the need for any additional parameterization.
In our work, we similarly employ the LLM-as-Optimizer approach when designing LLM-based Neurosymbolic Programs.


==> 3_2_method_algo_nsp_version_old.tex <==
\section{LLM-based Neurosymbolic Program - Declaration and Learning Algorithm}
\label{sec.method.algo}
\input{Figures/pipeline/inference}
Building on the connections made between LLM prompting and ERM framework in the previous section, we introduce the declaration and learning algorithms for constructing LLM-based Neurosymbolic Programs.
Section~\ref{sec.method.algo.definition} discusses how to present a Neurosymbolic Programs with LLMs.




\subsection{Preliminaries on Neurosymbolic Programs}
\wrc{review previous, then we add LLm with prompting module. This considers the simplest version: LLM + if-else}
\paragraph{Context-Free Gramma}
The space of Neurosymbolic Programs is often defined by a Context-Free Grammar, which includes a wide range of manually designed modules with various functions.
These modules can be combined into different models in tree-like structures known as Computation Graphs.
Figure~\ref{fig.nsp} shows an example gramma for sequential classification used in NEAR (cite).


\paragraph{Co-optimization of program structure and NN modules}
To learn a differentiable program, one needs to induce the program’s “architecture” while simultaneously optimizing the parameters of the program’s modules.
The complexity of this co-design task increases exponentially as the size of Context-Free Gramma expands, which are often necessary in order for the search space to cover more diverse programs.
To reduce the search cost, various learning algorithms have being proposed, including tree search (cite MC-NEAR, ) and continuous relaxation (cite NEAR, dPAD).


\paragraph{Trade-off between interpretability and expressiveness}
Modules in context-free gramma can be grouped into two categories:
(1). Symbolic modules, such as 'if-then-else,' 'map,' and 'sel.' These modules are human-interpretable but cannot define complex functions.
(2). Neural modules, exemplified by 'NN(x),' which are highly expressive yet operate as blackbox predictors.
This dichotomy presents an inherent dilemma for NSPs between interpretability and expressiveness. Incorporating more symbolic modules makes the decision-making process more transparent.
Conversely, using more neural modules enhances expressiveness.
Balancing interpretability and expressiveness in the learned program often involves incorporating human prior knowledge by assigning different costs to each type of module.

\begin{figure}[h]
    \centering
    \[
    \alpha ::= x \mid c \mid \bigoplus(\alpha_1, \ldots, \alpha_k) \mid \bigoplus_\theta(\alpha_1, \ldots, \alpha_k) \mid \text{if } \alpha_1 \text{ then } \alpha_2 \text{ else } \alpha_3 \mid \texttt{sel}_{\texttt{S}} x
    \]
    \[
    \texttt{map} (\texttt{fun } x_1.\alpha_1) \, x \mid \texttt{fold} (\texttt{fun } x_1.\alpha_1) \, c \, x \mid \texttt{mapprefix} (\texttt{fun } x_1.\alpha_1) \, x
    \]
    
    \caption{Example Grammar of DSL for sequence classification defined by NEAR and dPAD (cite). Here, $x$, $c$ represent inputs and constraints. $\bigoplus$ and $\bigoplus_\theta$ include a set of basic algebraic operations (e.g. \texttt{add}(), \texttt{multiply}(), \texttt{divide}()), and parameterized library functions (e.g. \texttt{nn}(x), \texttt{rnn}(x)), respectively. $\texttt{fun } x.e(x)$ represents an anonymous function that evaluates an expression $e(x)$ over the input $x$. $\texttt{sel}_{\texttt{S}}$ returns a vector consisting of a subset $S$ of the dimensions of an input $x$.}
    \label{fig.nsp}
\end{figure}

In the next section, we will show how pretrained LLMs can be leveraged to implement most modules in DSLs, thereby implementing NSPs that are both expressive and interpretable.
We show this by making a connection of LLM prompting with model selection, and show that they can represent a diverse set of powerful models via writing different instructions.




\subsection{Learning Theory of Prompting LLMs}
\wrc{TODO shorten this section}
\input{3_1_method_framework}



\subsection{Implementing Neuro-symbolic Programs with LLMs}
\label{sec.method.algo.definition}
\wrc{TODO: need to define those operators (input, output) better, currently it lacks consistency and clarity.}
\wrc{TODO: how to represent Sequential Program as a simplification/special case of Tree-based Programs}

By harnessing the capabilities of large language models (LLMs) in representing a wide range of functions via different prompts, we can significantly streamline the Grammar required to build traditional NSPs.
Specifically, for predictive models, the Grammar can be reduced to just three components: the input, conditional branching, and an LLM module. The formula is as follows:
\begin{align}
    % \alpha &::= x \mid \text{if } \alpha_1 \text{ then } \alpha_2 \text{ else } \alpha_3 \mid \texttt{LLM} (x, t),
    \alpha &::= x \mid \text{if } \alpha_1 \text{ then } \alpha_2 \text{ else } \alpha_3 \mid \texttt{LLM} (x, t).
    \label{eq:cfg.lsp}
\end{align}
Here, $\texttt{LLM}(x, t)$ refers to the response from the LLM given the input $x$ and the instruction $t$.
Furthermore, we can combine the conditional branching and the LLM module into a single component to simplify the grammar even more.
In the structure of the program, each component can contain all other components as children.
This allows us to merge components:
(1) For the conditional branching, if its inputs are popularized by another branching operator, we can combine them by linking their conditions;
(2) For the LLM module, if its input $x$ is popularized by another LLM module, we can merge them through sequential prompting in a conversational flow."
The final simplified grammar for predictive modeling is as follows:
\begin{align}
    % \alpha &::= x \mid \texttt{switch}(\texttt{LLM} (x, t)).
    \alpha ::= x \mid \texttt{switch}(\texttt{LLM}(x, t), \{ y_i: \alpha_i \}_{i=1}^{k})
    \label{eq:cfg.lsp.simplified}
\end{align}
Here, the function $\texttt{switch}(\texttt{LLM}(x, t), \{ y_i: \alpha_i \}_{i=1}^{k})$ directs program execution to one of the sub-programs, $\alpha_i$, based on the output, $y_i$, from $\texttt{LLM}(x, t)$.
Figure~\ref{fig:inference} shows an example LLM-Symbolic Program discovered from the above Grammar.
Given a test query, the inference process traverses the tree-structured program in a top-down order.
The data will be assigned to a specific child node based on the parent node's decisions, until the leaf node with final output is reached.

\paragraph{Remark: can LLMs implement the conditional branching?}
In our final grammar (referenced as Gramma~\ref{eq:cfg.lsp.simplified}), we choose to define the conditional branching operator separately rather than incorporating it within the LLM.
This decision is based on the fact that while LLMs can theoretically handle tree data, they are currently prone to hallucinations in processing them natively (cite).
Since conditional branching is a simple well-defined deterministic function, using it directly helps avoid unnecessary errors and maintains the reliability of the program.
This approach is similar to the Tree-of-Thought method, where the process of expanding the solution tree is implemented outside of LLMs.
This is despite LLMs' ability to somewhat replicate various tree-search algorithms (cite).






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Learning algorithm for LSPs}
\label{sec.method.algo.definition}


\paragraph{Co-optimization of program structure and parameterized operators}
The adoption of LLM not only simplifies the program declaration, but also makes their learning more tractable.
In traditional NSPs, searching the optimal program structure over a complex CFG space with multiple opeartor is a combinatorial optimization problem where candidate evaluations are expensive: the parameters for each NN-operators must be optimized from scratch every time a new structure is proposed.

For LLM-Symbolic Programs, since the Grammar consists of only two operators (input and LLM module), expanding the program structures can be accomplished via simple top-down tree traversal, where a wide range of well-established search algorithms applies, such as A* search, DFS/BFS, MCTS, etc.
Here, we adopt A* as an example to layout our complete learning pipeline, but also experiment with two other well-established search algorithms: BFS and MCTS in later analysis.
For A* search, the only remaining questions to address are (1). training each LLM module (2). a score function for each node to guide the search algorithm.
The complete search process is illustrated in Figure~\ref{fig.astar} and detailed in Algorithm~\ref{algo.astar}.
\wrc{insert an algorithm box here}


\paragraph{Learning LLM module by summarizing rules}
In the structured setup of a program, each LLM module is responsible for making decisions on the subset of data it receives.
In traditional NSPs, the learnable NN modules are usually trained using empirical risk minimization, which is closely linked to prompt optimization, as previously established.
This essentially transforms the training process into deriving instructions from observed data.
Recent advancements in prompt optimization take advantage of the LLM's ability to deduce task descriptions directly from data or to enhance human-written prompts based on prediction errors.
However, we adopt a more straightforward approach that utilizes the LLM’s more robust summarization capabilities, asking the model to directly generate predictive rules they observe from the data.
This method uses a 'meta prompt' strategy, as shown in Figure~\ref{fig.meta_prompt}, where the LLM first identifies patterns in the examples provided and then formulates these observations into a coherent set of rules.
% The key idea for constructing LSP is to progressively expand the program structure and find the right prompt for each newly added LLM operands.
% Since all programs built on top of DSL have tree structures, most graph search heuristics can be extended to accomplish this task.
% Here, we adopt A* as an example to layout our complete learning pipeline, but also experiment with two other well-established search algorithms: BFS and MCTS in later analysis.


\paragraph{Scoring function for each node}
Most top-down tree search algorithms, including A*, require a node scoring function to decide which node to expand next.
In our case, the leaf nodes of the program return final predictions on the input data, making error metrics like total errors a natural choice for scoring.
We specifically use the total number of errors to score each leaf node because this absolute metric takes into account the size of the data subset each node processes.
Additionally, empirical evidence suggests that counting errors tends to be more reliable than other metrics such as accuracy or LLM-based scores, as ablated in Section~\ref{sec.ablate.scorer}.

\wrc{issue: Formally, A* requires an admissible heurisitic, not just any score function. I'll try to frame this into an approximately admissible heuristic}
% \paragraph{Approximatedly-Admissible Heuristic for A* search}
% A* search guarantees the optimal solution with Admissible Heuristic.
% However, if the heuristic is approximately admissible, A* search is still able to converge to a good enough solution.


\subsection{Benefits of LSP}
\label{sec.method.algo.benefit}
comparing with XAI methods (linear model, decision tree, NSP) and Vanilla Prompting
\begin{itemize}
    \item Compare with conventional XAI methods, LSPs are expressive and interpretable.
    \item comparing with NSP that requries customizing DSLs for every task (cite), LSP can be optimized on any tasks with minimal human intervention.
    \item generalizable: since learned instructions are natural language, they are human readable and robust to distribution shift (such as image variations).
    \item Comparing with tuning prompts for LLMs as a whole, the tree-structured LSPs solve the problem via divide and conquer, each node will only need to summarize the subset of dataset assigned to it. This simplifies the instruction learning and following process, resulting in better predictors.
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%










% \subsection{(Tentative) Other techniques worth mentioning here}
% \begin{itemize}
%     \item error selection (if this is the only one, then move it to 3.2/3.3)
%     \item Chain-of-thought summarization
% \end{itemize}


% \subsection{Can LLMs directly operate on structured prompts?}
% \begin{itemize}
%     \item We explicitly manages the data structure and their corresponding operations, a natural question is can we outsource this to LLM as well, via prompting?
%     \item If the model is good enough then yes, but current models often cannot do this.
% \end{itemize}


==> Figures/pipeline/dsl_near.tex <==
% \begin{figure}[h]
%     \centering
%     % \[
%     % \alpha ::= x \mid c \mid \bigoplus(\alpha_1, \ldots, \alpha_k) \mid \bigoplus_\theta(\alpha_1, \ldots, \alpha_k) \mid \text{if } \alpha_1 \text{ then } \alpha_2 \text{ else } \alpha_3 \mid \texttt{sel}_{\texttt{S}} x
%     % \]
%     \[
%         \textbf{DSL:} \quad
%         \alpha ::= x \mid \bigoplus{\{\alpha_i\}}_{i=1}^k \mid
%         \bigoplus_\theta{\{\alpha_i\}}_{i=1}^k \mid
%         \text{if } \alpha_1 \text{ then } \alpha_2 \text{ else } \alpha_3 \mid
%         \texttt{map} (\texttt{fun } x_1.\alpha_1) \mid
%         \cdots
%     \]
%     \[
%         \textbf{Program:} \quad
%         \texttt{map} \ (\texttt{fun} \ x_t.
%         \ \texttt{if} \ \text{DistAffine}(x_t)
%         \ \texttt{then} \ \text{AccAffine}(x_t)
%         \ \texttt{else} \ \text{DistAffine}(x_t)) \ x
%     \]
%     \caption{
%         \textbf{\sisi{since this is very long, how about we have a paragraph in the main text to explain the concept?}Top: DSL for sequence classification task defined in NEAR\sisi{citation}}. Here, $x$ represent inputs \sisi{define what is $a_i$}; $\bigoplus$ and $\bigoplus_\theta$ \felix{this is a bit confusing. what is the difference between $\bigoplus$ and $\bigoplus$ with $\theta$?}\sisi{what is $\theta$ for in the equation.} include a set of basic algebraic operations (e.g. \texttt{add}(), \texttt{multiply}(), \texttt{divide}()), and parameterized operators (e.g. \texttt{nn}(x), \texttt{rnn}(x)), respectively. $\texttt{fun } x.e(x)$ represents an anonymous function that evaluates an expression $e(x)$ over the input $x$.
%         \textbf{Bottom: Synthesized program classifying a sniff action between two mice in the CRIM13 dataset\sisi{citation}.} Weights for the affine operators are omitted for simplicity. Here, DistAffine and AccAffine are manually designed neural feature extractor modules belonging to $\bigoplus_\theta$. The program can be interpreted as follows: if the distance between two mice is small, they are doing a sniff (large bias in else clause). Otherwise, they are doing a “sniff” if the difference between their accelerations is small. Captions borrowed from Figure 1 \& 2 in the original NEAR paper (cite)\sisi{are all these borrowed from the paper even Figure 1? I think we need to rewrite things. It is fine to use the same equation, but we need to have our way to explain things, it is not good to just copy everything from a previous paper.}. \sisi{questions: is above equation 1 and equation 2 related? or these two are two forms of DSL? I feel the caption is not very clear. Maybe let us have a long paragraph to explain it?}
%         \cho{How about we just create a simple NSP as the example here? }
%         \wrc{I'll simplify the prelim section.}
%     }
% \label{fig:dsl_near}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \[
%         \textbf{DSL:} \quad
%         \alpha ::= x \mid c
%         \mid \texttt{Add}(\alpha_1, \alpha_2) \mid \texttt{Mul}(\alpha_1, \alpha_2)
%         \mid \text{If } \alpha_1 \text{ Then } \alpha_2 \text{ Else } \alpha_3
%         \mid \texttt{cnn}(x, \theta) \mid \texttt{Dist}(\alpha_1, \alpha_2)
%         % \cdots
%     \]
%     \[
%         \textbf{Program:} \quad
%         \texttt{map} \ (\texttt{fun} \ x_t.
%         \ \texttt{if} \ \text{DistAffine}(x_t)
%         \ \texttt{then} \ \text{AccAffine}(x_t)
%         \ \texttt{else} \ \text{DistAffine}(x_t)) \ x
%     \]
%     \caption{
%         \textbf{Top: Example Domain-Specific Language}. Here, $x$ represent inputs and constants and $\alpha$ are sub-programs.
%         \textbf{Bottom: Synthesized program classifying a  dataset\sisi{citation}.}
%     }
% \label{fig:dsl_near}
% \end{figure}

==> Tables/exp_settings.tex <==
\begin{table}[t!]
\tiny
\centering
\caption{Exp Settings}

\resizebox{0.92\textwidth}{!}{
    \begin{tabular}{p{2cm}p{8cm}}
    
    \toprule
    \textbf{Dimension} & \textbf{Options} \\
    \midrule
    \midrule
    \textbf{Modalities} & \texttt{Text,} \ \texttt{Vision} \\
    \midrule
    \textbf{Optimizer-Models} & \texttt{GPT3.5,} \ \texttt{GPT4,} \ \texttt{GPT4-Vision,} \ \texttt{Gemini-1.0,} \ \texttt{Gemini-1.0-Vision} \\
    \midrule
    \textbf{Predictor-Models} & \texttt{GPT3.5,} \ \texttt{GPT4-Vision,} \ \texttt{Gemini1.0,} \ \texttt{Gemini1.0-Vision} \\
    \midrule
    \textbf{Baselines} & \texttt{Monte Carlo,} \ \texttt{Evolutionary Search,} \ \texttt{Beam Search,} \ \texttt{Tree Search} \\
    \midrule
    
    \bottomrule
    \end{tabular}
}
\label{table:exp_settings}
\end{table}

==> Tables/main_exp.tex <==
% \begin{table}
%   \caption{Classification accuracy comparison with other methods on Text Benchmarks (will turn it into a Figure)}
% %   \label{tab:main_exp}
%   \centering
%   \resizebox{1\textwidth}{!}{
%   \begin{tabular}{cc|c|cc|ccccccc}
%     \toprule
    
%     \midrule
%     Text Benchmark & 
%     & \multicolumn{1}{c}{Synthetic}
%     & \multicolumn{2}{c}{NLP}
%     & \multicolumn{6}{c}{Caption} \\
%     \midrule
%     & Method
%     & Decision Tree
%     & Ethos & Liar
%     & Waxwing & Waterthrush & Jaeger & Albatross & Blackbird & Swallow \\
%     \midrule
    
%     \multirow{7}{*}{GPT-3.5-Turbo}
%         & RAW
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & APE
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & PromptAgent
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & APO
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & List
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & Tree
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         % \cmidrule(r){2-11}
%     \midrule

%     \multirow{7}{*}{Gemini-1.0-Pro}
%         & RAW
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & APE
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & PromptAgent
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & APO
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & List
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         \cmidrule(r){2-11}
%         & LSP (Ours)
%         & $\pm$
%         & $\pm$ & $\pm$
%         & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ & $\pm$ \\
%         % \cmidrule(r){2-11}
%     \midrule
    
%     \bottomrule

%   \end{tabular}
%   }
% \end{table}

